Predicting Scheduling Failures in the Cloud

Cloud Computing has emerged as a key technology to deliver and manage computing, platform, and software services over the Internet. Task scheduling algorithms play an important role in the efficiency of cloud computing services as they aim to reduce the turnaround time of tasks and improve resource utilization. Several task scheduling algorithms have been proposed in the literature for cloud computing systems, the majority relying on the computational complexity of tasks and the distribution of resources. However, several tasks scheduled following these algorithms still fail because of unforeseen changes in the cloud environments. In this paper, using tasks execution and resource utilization data extracted from the execution traces of real world applications at Google, we explore the possibility of predicting the scheduling outcome of a task using statistical models. If we can successfully predict tasks failures, we may be able to reduce the execution time of jobs by rescheduling failed tasks earlier (i.e., before their actual failing time). Our results show that statistical models can predict task failures with a precision up to 97.4%, and a recall up to 96.2%. We simulate the potential benefits of such predictions using the tool kit GloudSim and found that they can improve the number of finished tasks by up to 40%. We also perform a case study using the Hadoop framework of Amazon Elastic MapReduce (EMR) and the jobs of a gene expression correlations analysis study from breast cancer research. We find that when extending the scheduler of Hadoop with our predictive models, the percentage of failed jobs can be reduced by up to 45%, with an overhead of less than 5 minutes.

==> threat.tex <==
\section{Threats to Validity}
\label{sec:threats}
This section discusses the threats to validity of our study following the guidelines for case study research~\cite{robert2002case}.

\emph{\textbf{Construct validity threats}} concern the relation between theory and observation. Our modelling approach assumes that tasks and jobs characteristics alone can explain scheduling outcomes, when in reality, this may not be the case. It is possible that other factors such as scheduling class or resources allocation strategy also play a role in scheduling decisions. However, in our data set we found a low correlation between scheduling class and scheduling outcomes. According to ~\cite{[8]}, this low correlation is due to the fact that the scheduling class which represents the latency-sensitivity of a task/job mostly affects local machine policies for accessing cluster resources. They are therefore more likely to affect resource usages than scheduling outcomes. Also, in our data set, assigned resources were too high compared to the requested resources (this is explained by the overbooking strategy adopted by Google ~\cite{[16]}) nullifying the impact of resource allocation on scheduling outcomes. Also, our modelling did not considered task constraints, which specify the machines on which a task can run. In future work, we plan to examine the relation between task constraints and scheduling outcomes. 
%In future work we plan to investigate.....\Foutse{complete?}.
%
Another construct validly threat concerns the size of the data set on which our results are obtained (we randomly sampled 2\% of tasks and jobs contained in the Google data set). However, since we obtained consistent results for different samples of the same Google data set, we are confident that our findings can hold on the whole Google data set. %ur data sampling.
We analyzed only 2\% of tasks files contained in the Google dataset. However, to ensure that our findings hold for the remaining dataset, we collect 10\% additional sample from the same dataset and obtained the same results.
%have verify our results on multiple samples resampled

\textbf{\emph{Internal validity threats}} concern our selection of subject systems, tools, and analysis method. Although the Google data set used in this study may not contain all the different kinds of task and jobs used in the industry, it represents the execution of real applications from a major company (i.e., Google). The GloudSim scheduler used in \textbf{RQ3} does not represent of all existing schedulers in the industry. However, it is designed to reproduce the scheduler used in some Google clusters. Moreover, the tool kit GloudSim has already been used successfully in many research projects ~\cite{[25]} ~\cite{[26]} .



\textbf{\emph{Conclusion validity threats}} concern the relation between the treatment and the outcome. We paid attention not to violate assumptions of the constructed statistical models.


\textbf{\emph{Reliability validity threats}} concern the possibility of replicating this study. Every result obtained through empirical studies is threatened by potential bias from data sets \cite{menzies2007data}. We provide all necessary details needed to replicate our study. The Google data set is publicly available for study.

\textbf{\emph{External validity threats}} concern the possibility to generalize our results. Our study is based on large-scale data (i.e., \textit{158 GB}) collected from Google clusters. Nevertheless, further validation on larger and diverse sets of tasks and jobs is desirable.



